PPTBench: Towards Holistic Evaluation of Large Language Models for PowerPoint Layout and Design Understanding

PowerPoint presentations combine rich textual content with structured visual layouts, making them a natural testbed for evaluating the multimodal reasoning and layout understanding abilities of modern MLLMs. However, existing benchmarks focus solely on narrow subtasks while overlooking layout-centric challenges, which are central to real-world slide creation and editing. To bridge this gap, we introduce PPTBench, a comprehensive multimodal benchmark for evaluating LLMs on PowerPoint-related tasks. Leveraging a diverse source of 958 PPTX files, PPTBench evaluates models across four categories with 4,439 samples, including Detection, Understanding, Modification, and Generation. Our experiments reveal a substantial gap between semantic understanding and visual-layout reasoning in current MLLMs: models can interpret slide content but fail to produce coherent spatial arrangements. Ablation and further analysis show that current MLLMs struggle to combine visual cues with JSON-based layout structures and fail to integrate visual information into their API planning ability. And case studies visually expose systematic layout errors such as misalignment and element overlap. These findings provides a new perspective on evaluating VLLMs in PPT scenarios, highlighting challenges and directions for future research on visual-structural reasoning and coherent slide generation. All datasets and code are fully released to support reproducibility and future research.

==> sec/6_limitations.tex <==
\section{Limitations and Future Work}

While PPTBench provides a comprehensive framework for evaluating LLMs on PowerPoint-related 
tasks, we acknowledge several limitations and identify promising directions for future research:

\paragraph{Dataset Limitations.}
Our current dataset primarily consists of 958 government PowerPoint presentations, focusing 
on public health, education, and science domains in English. This limited scope may not 
fully capture the diversity of real-world presentations across different:
\begin{itemize}
    \item \textbf{Domains:} Business presentations, academic lectures, and creative 
    portfolios may exhibit different patterns and requirements
    \item \textbf{Languages:} Multi-lingual support is crucial for global applications
    \item \textbf{Cultural contexts:} Presentation styles and conventions vary across regions 
    and industries
\end{itemize}

\paragraph{Technical Constraints.}
Several technical aspects warrant further investigation:
\begin{itemize}
    \item \textbf{Format coverage:} Our dataset predominantly uses the 4:3 aspect ratio, 
    while modern presentations typically use 16:9 widescreen format
    \item \textbf{Dynamic elements:} Current evaluation excludes slide transitions, 
    animations, and interactive elements that are common in professional presentations
    \item \textbf{Media types:} Limited coverage of advanced features like embedded 
    videos, audio elements, and interactive charts
\end{itemize}
